Vision Transformers provably learn spatial structure

Vision Transformers (ViTs) have achieved comparable or superior performance than Convolutional Neural Networks (CNNs) in computer vision. This empirical breakthrough is even more remarkable since, in contrast to CNNs, ViTs do not embed any visual inductive bias of spatial locality. Yet, recent works have shown that while minimizing their training loss, ViTs specifically learn spatially localized patterns. This raises a central question: how do ViTs learn these patterns by solely minimizing their training loss using gradient-based methods from random initialization? In this paper, we provide some theoretical justification of this phenomenon. We propose a spatially structured dataset and a simplified ViT model. In this model, the attention matrix solely depends on the positional encodings. We call this mechanism the positional attention mechanism. On the theoretical side, we consider a binary classification task and show that while the learning problem admits multiple solutions that generalize, our model implicitly learns the spatial structure of the dataset while generalizing: we call this phenomenon patch association. We prove that patch association helps to sample-efficiently transfer to downstream datasets that share the same structure as the pre-training one but differ in the features. Lastly, we empirically verify that a ViT with positional attention performs similarly to the original one on CIFAR-10/100, SVHN and ImageNet.

==> transfer.tex <==
\section{Patch association yields sample-efficient fine-tuning with ViTs}\label{sec:transfer}

%%We examine a downstream dataset $\mathring{S}=\{(\widetilde{\bm{X}}^{(i)},\Tilde{y}^{(i)}\}_{i=1}^{\tilde{N}}$ sampled from the distribution  $\widetilde{\mathcal{D}}$ where the data-points share a \textit{similar} structure as $\mathcal{D}$ but with a \textit{different} feature $\widetilde{\bm{w}}^*.$ The generative process of $\widetilde{\mathcal{D}}$ is similar to the one of $\mathcal{D}$ except the following steps: 

A fundamental byproduct of our theory is that after pre-training on a dataset sampled from $\mathcal{D}$, our model  \eqref{eq:transformer} sample-efficiently transfers to datasets that are structured as $\mathcal{D}$ but differ in their features.

\vspace*{-.4cm}
\paragraph{Downstream dataset.} Let $\widetilde{\mathcal{D}}$ a downstream data distribution  defined as in \autoref{def:datadist} such that its underlying feature is $\widetilde{\bm{w}}^*$ with $\|\widetilde{\bm{w}}^*\|_2=1$ and $\widetilde{\bm{w}}^*$ potentially different from $\bm{w}^*$. In other words, the downstream $\widetilde{\mathcal{D}}$ and source $\mathcal{D}$ distributions share the same structure but not necessarily the same feature. We sample a downstream dataset $\widetilde{\mathcal{Z}}=\{(\widetilde{\bm{X}}[i],\widetilde{y}[i])\}_{i=1}^{\widetilde{N}}$ from $\widetilde{\mathcal{D}}$.


%$\widetilde{\bm{w}}^*\in\mathbb{R}^d$ such that $\|\widetilde{\bm{w}}^*\|_2=1$ and  $\{\widetilde{\bm{\xi}}_j\}_{j=1}^D$ be such that $\widetilde{\bm{\xi}}_i\sim\mathcal{N}(0,\sigma^2\mathbf{I}_d).$ Let  $\{\widetilde{\delta}_j\}_{j=1}^D$ be a collection of random variables such that $\widetilde{\delta}_j=1$ with probability $q/2$, $\widetilde{\delta}_j=-1$ with the same probability and $0$ otherwise. The downstream distribution $\widetilde{\mathcal{D}}$ follows the same generative process as $\mathcal{D}$ except for the following steps:  
%\begin{enumerate}
% \setcounter{enumi}{3}
%    \item  \textbf{Signal set}: for $i\in\mathcal{S}_{\ell(\bm{X})}$, $ \bm{X}_i=y\widetilde{\bm{w}}^*+\widetilde{\bm{\xi}}_i$.
    %%%%, where $\widetilde{\bm{\xi}}_i\sim\mathcal{N}(0,\sigma^2\mathbf{I}_d).$
%    \item \textbf{Random set}: for $j\in\mathcal{S}_{\ell}$ with $\ell\neq\ell(\bm{X})$, $\bm{X}_j=\widetilde{\delta}_{j}\widetilde{\bm{w}}^*+\widetilde{\bm{\xi}}_{j}$.
    %%%%, where $\widetilde{\delta}_{j}=1$ with probability $q/2$, $-1$ with the same probability and $0$ otherwise and $\widetilde{\bm{\xi}}_{j}\sim\mathcal{N}(0,\sigma^2\mathbf{I}_d).$
%\end{enumerate}
%Using this process, we generate a downstream dataset $\widetilde{S}=\{(\widetilde{\bm{X}}[i],\widetilde{y}[i]\}_{i=1}^{\widetilde{N}}$.

\vspace*{-.4cm}


\paragraph{Learning problem.} We consider the model \eqref{eq:transformer} pre-trained as in  \autoref{sec:theory_real}. We assume that $\widehat{\bm{A}}$ is  kept \textit{fixed} from the pre-trained model and we only optimize the value vector $\widetilde{\bm{v}}$ to solve:

\vspace{-.8cm}

\begin{align}\label{eq:empirical_transfer}\tag{$\widetilde{\text{E}}$}
    \min_{\widetilde{\bm{v}}}\;\; \frac{1}{\widetilde{N}}\sum_{i=1}^{\widetilde{N}} \log\big(1+e^{-\widetilde{y}[i]F(\widetilde{\bm{X}}[i])}\big):=\widetilde{\mathcal{L}}(\widetilde{\bm{v}}).
\end{align}

\vspace{-.4cm}


We run GD on \eqref{eq:empirical_transfer} with parameters set as in \autoref{param} except that the $\widehat{A}_{i,j}$'s are fixed and $\widetilde{\bm{v}}^{(0)}\sim\mathcal{N}(0,\omega^2\mathbf{I}_d)$ with $\omega=1/\mathrm{poly}(d)$. Our main results states that this fine-tuning procedure requires a few samples to achieve high test accuracy in $\widetilde{\mathcal{D}}$. In contrast, any algorithm without patch association needs a large number of samples to generalize.
%Our main result states that this fine-tuning procedure requires a few samples to achieve high test accuracy in $\widetilde{\mathcal{D}}$. %[Sample efficient adaptation with pre-training]
\begin{restatable}{theorem}{thmtransfer}\label{thm:transfer}
 Let $\widehat{\bm{A}}$ be the attention matrix obtained after pre-training as in \autoref{sec:theory_real}. Assume that we run GD for $T$ iterations on \eqref{eq:empirical_transfer} to  fine-tune the value vector. Using $\widetilde{N}\leq\mathrm{polylog}(D)$ samples, the model \eqref{eq:transformer} transfers to $\widetilde{\mathcal{D}}$ i.e.\ $\mathbb{P}_{\widetilde{\mathcal{D}}}[f^*(\bm{X})F_{\widehat{\bm{A}},\widetilde{\bm{v}}^{(T)}}(\bm{X})>0]\geq 1-o(1).$
\end{restatable}
 \begin{proof}[Proof of \autoref{thm:transfer}]
Actually, even one step of the update using normalized gradient descent on $\bm{v}$ can already achieve test accuracy $\geq 1-o(1).$ We know that for a datum $(\bm{X}, y)$, the gradient of $L(\bm{X})$ with respect to $\bm{v}$ is
\begin{align}\label{eq:grad_trf}
    \nabla_{\bm{v}}L(\bm{X})=-y\mathfrak{S}(-yF(\bm{X}))\sum_{m=1}^D \sigma'(\langle\bm{O}_m^{(t)},\widetilde{\bm{v}}^{(t)}\rangle)\bm{O}_m^{(t)}
\end{align}
Since $\widetilde{\bm{v}}^{(0)}=\bm{0},$ we have $F_{\widetilde{\bm{v}}^{(0)}}(\bm{X})=0$ and $\sigma'(\langle\bm{O}_m^{(0)},\widetilde{\bm{v}}^{(0)}\rangle)=\nu.$ Thus, the gradient \eqref{eq:grad_trf} simplifies to
\begin{align}
     \nabla_{\bm{v}}L(\bm{X})= -\frac{\nu y}{2}\sum_{j=1}^D\bm{X}_j\sum_{m=1}^D \widehat{S}_{m,j}^{(t)}
\end{align}
By symmetry of the $\widehat{S}_{j,m}^{(t)}$  , we know that
\begin{align}
    \Big|\sum_{m=1}^D \widehat{S}_{m,j}^{(t)} -D\Big|\leq \frac{D}{\mathrm{poly}(d)},
\end{align}
where $\frac{1}{\mathrm{poly}(d)}$
comes from the $\varepsilon_{\bm{Q}}$ part in the previous section. Moreover, since the noise and feature noise has mean zero independent of $y$, we know that there
exists some value $c_0>0$ (roughly equal to $\alpha DC$) ) such that:
\begin{align}
    \mathbb{E}[ \nabla_{\bm{v}}L(\bm{X})]&= c_0 \widetilde{\bm{w}}^*.
\end{align}
Now, by standard concentration inequality, we know that for $N$ i.i.d. samples $\bm{X}[i],y[i]$, with high probability
\begin{align}
    \bm{\nabla}_0:=\sum_{i=1}^N \nabla_{\bm{v}}L(\bm{X}[i])=c_0 \widetilde{\bm{w}}^* +\varepsilon_0\widetilde{\bm{w}}^*+\bm{\chi}_{0},
\end{align}
where $\varepsilon_0$ comes from the feature noise
\begin{align}
    |\varepsilon_0|\leq \frac{c_0 qD\log(d)}{\sqrt{N}},
\end{align}
and $\bm{\chi}_{0}$ comes from the noise:
\begin{align}
    \|\bm{\chi}_{0}\|_2\leq\frac{c_0\sigma\sqrt{d}\sqrt{D}}{\sqrt{N}}.
\end{align}
Therefore, if we update using normalized GD:
\begin{align}
    \widetilde{\bm{v}}^{(1)}&=\widetilde{\bm{v}}^{(0)}+\frac{\bm{\nabla}_0}{\|\bm{\nabla}_0\|_2}
\end{align}
we have that:
\begin{align}
    \widetilde{\bm{v}}^{(1)}&= c_1 \widetilde{\bm{w}}^*+\bm{\chi}_{1},
\end{align}
where $\bm{\chi}_{1}\perp\widetilde{\bm{w}}^*$, $\|\bm{\chi}_{1}\|_2=O(1)$ and $c_1\geq \Tilde{\Omega}(1)/\sqrt{D}.$ Now, for a new datum $\bm{X}^{new}$ with noises $\{\bm{\xi}_i^{new}\}_{i=1}^D$, we know that w.h.p
\begin{align}
    |\langle \bm{\xi}_i^{new},\widetilde{\bm{v}}^{(1)}\rangle|\leq\frac{\Tilde{O}(1)}{\sqrt{d}}, \qquad |\langle \widetilde{\bm{w}}^{*},\widetilde{\bm{v}}^{(1)}\rangle| \geq \frac{\Tilde{\Omega}(1)}{\sqrt{D}}.
\end{align}
We can prove the test accuracy is small using the same proof as in  \autoref{lem:cv_pop}, where we show
that:
\begin{align}
    y\sigma(\langle  \widetilde{\bm{v}}^{(1)}, \bm{O}_m^{(1)}\rangle)\geq 0,
\end{align}
for $m\in\mathcal{S}_{\ell(\bm{X})}$  and it dominates the other $ y\sigma(\langle  \widetilde{\bm{v}}^{(1)}, \bm{O}_j^{(1)}\rangle)$ for $j\in\mathcal{S}_{\ell}$ with $\ell\neq\ell(\bm{X}).$  Therefore, we prove that $\mathbb{P}_{\widetilde{\mathcal{D}}}[yF(\bm{X})>0]\geq 1-o(1)$ which implies the aimed result.
\end{proof}
% During the optimization, we have $\widetilde{\bm{v}}^{(t)} = \widetilde{\alpha}^{(t)}\widetilde{\bm{w}}^*+\widetilde{\varepsilon}_{\bm{v}}^{(t)}\widetilde{\bm{u}}^{(t)}.$ The dynamics of $\widetilde{\bm{v}}$ is similar to the one of $\hat{\bm{v}}$ in \autoref{sec:theory_real}. Therefore, \autoref{lem:event3} and \autoref{lem:epsv} respectively provide a bound on $\widetilde{\alpha}^{(t)}$ and $\widetilde{\varepsilon}_{\bm{v}}^{(t)}.$ We finally resort to classical generalization bounds based on the Rademacher complexity to obtain the sample complexity in \autoref{thm:transfer}. 

%any algorithm without pre-training or prior knowledge of the underlying structure

\begin{restatable}{theorem}{thmtransfernegative}\label{thm:samplcomplexA}
 Let $\mathcal{A}\colon\mathbb{R}^{d\times D}\rightarrow\{-1,1\}$ be a binary classification algorithm without patch association knowledge.  Then, it needs  $ D^{\Omega(1)}$ training samples to get test error $\leq o(1)$ on $\widetilde{\mathcal{D}}$. %$\mathbb{P}_{(\bm{X},y)\sim\widetilde{\mathcal{D}}}[y\mathcal{A}(\bm{X})>0]\geq 1-o(1).$
\end{restatable}

\begin{proof}[Proof of \autoref{thm:samplcomplexA}]
Let $\mathcal{A}$ be an algorithm.
Assume that at training time the algorithm $\mathcal{A}$ has access to $D^{o(1)}$ training data, Since each input $X$ is made of $D$ patches, this means that there exist at least $\Omega(1)$ fraction of $k\in[D]$ such that $\mathcal{A}$ has not seen training samples with $\ell(X)=k$. Consider the following two distributions over $\{-1, 0, 1\}^m$:
\begin{enumerate}
    \item  $\mathcal{D}_1$: Sample $z \in \{0, 1\}^m$ where each $z_i$ i.i.d. $1$ w.p. $q/2$, $-1$ w.p. $q/2$ and $0$ otherwise. 
    
    \item  $\mathcal{D}_2$: Sample a set $\mathcal{S}$ uniformly at random from $[m]$ of size $C$, set all $z_i = 1$ for $i \in \mathcal{S}$, and sample other $z_j$  i.i.d. $1$ w.p. $q/2$, $-1$ w.p. $q/2$ and $0$ otherwise. 
\end{enumerate}

We can easily see that as long as $qm = \text{poly}(C)$, then 
$$\textbf{TV}(\mathcal{D}_1, \mathcal{D}_2) = o(1)$$

This implies that $\mathcal{A}$ must have bad generalization error ($\Omega(1)$) on $\tilde{\mathcal{D}}$.


%Since $\ell(X)$ contains the label of the datapoint, this implies that  $\mathcal{A}$ cannot well generalize on test samples with $\ell(X)=k$. Therefore,  $D^{\Omega(1)}$ samples are at least needed to generalize.
\end{proof}

%\textcolor{red}{Intuitively, when an algorithm $\mathcal{A}$ is given less than $D^{\Omega(1)}$ training samples,   there exists some set $\mathcal{S}_{k}$ that $\mathcal{A}$ has not seen during training. Therefore, $\mathcal{A}$ cannot classify test samples such that $\ell(\bm{X})=k$ and thus incurs high generalization error.} \autoref{thm:transfer} and \autoref{thm:samplcomplexA} show that our model is sample-efficient for transfer. %without knowing the patch associations $\mathcal{S}_{\ell}$ as prior.
%The proofs of \autoref{thm:transfer} and \autoref{thm:samplcomplexA} are in \autoref{sec:app_transfer}. 
These theorems highlight that learning patch association is required for efficient transfer. We believe that they offer a new perspective on explaining why ViTs are widely used in transferring to downstream tasks. While it is possible that ViTs learn shared (with the downstream dataset) features during pretraining, our theory hints that learning the inductive bias of the labeling function is also central for transfer.






%Our theory differs from prior theoretical results in transfer learning for two reasons. Many of these works \citep{baxter00,maurer15,tripurameni2020} consider a downstream dataset that shares some features with the pre-training dataset. During transfer, they freeze their models' representations and learn a linear combination of these latter. In our case, the features in the downstream dataset may be totally independent from the pre-training one. Therefore, we rather learn new representations from scratch. We believe that this is more representative to what is done in practice as practicioners usually fine-tune their models. More importantly, our theory offers another view on transfer when using transformers. While knowing some shared features may help, we show here that a model having the knowledge on the underlying structure of the downstream may be key to explain why transformers efficiently transfers. This observation may be confirmed by works showing that ViTs transfer better than CNNs to downstream datasets with major distribution shift \citep{zhang2021}.

%how transformers sample-efficiently transfers. Contrary to several works in transfer learning, our model does not transfer because it previously learned some shared features/representations \citep{baxter00,maurer15} but mainly because it already learned the underlying structure of the downstream dataset. 


%is mainly due to  the attention matrix learned the patch pairing map. transformers transfer is not because they learn the feature but rather the structure of the dataset. This aligns with the use of transformers that are trained on Imagenet and transfer to multiple and diverse image classification datasets  \citep{dosovitskiy2020image}.

%\textcolor{red}{Interesting result because we fine-tune (and not train the last layer as many papers) and this is what is done in practice. Hints that learning the structure is essential to transfer. This may explain why transformers are widely used in transfer learning because datasets share same structure but different features.}
 



